Speeding Up Multi-Objective Hyperparameter Optimization by Task Similarity-Based Meta-Learning for the Tree-Structured Parzen Estimator

Hyperparameter optimization (HPO) is a vital step in improving performance in deep learning (DL). Practitioners are often faced with the trade-off between multiple criteria, such as accuracy and latency. Given the high computational needs of DL and the growing demand for efficient HPO, the acceleration of multi-objective (MO) optimization becomes ever more important. Despite the significant body of work on meta-learning for HPO, existing methods are inapplicable to MO tree-structured Parzen estimator (MO-TPE), a simple yet powerful MO-HPO algorithm. In this paper, we extend TPE's acquisition function to the meta-learning setting using a task similarity defined by the overlap of top domains between tasks. We also theoretically analyze and address the limitations of our task similarity. In the experiments, we demonstrate that our method speeds up MO-TPE on tabular HPO benchmarks and attains state-of-the-art performance. Our method was also validated externally by winning the AutoML 2022 competition on "Multiobjective Hyperparameter Optimization for Transformers".

==> appendices/proofs/hp-importance.tex <==
\subsection{Proof of Proposition \ref{main:methods:proposition:hp-importance}}
\label{appendix:proofs:subsection:proof-of-hp-importance}
We first introduce the following marginal
mean of the binary function $b(\xv | \Xg)$ for the proof:
\begin{definition}[Marginal mean]
  \begin{equation}
    \begin{aligned}
      q(x_i | \Xg) \coloneqq \int_{\xv \in \X} b(\xv | \Xg) \frac{\mu(d\xv_{-i})}{\mu(\X_{-i})}
    \end{aligned}
  \end{equation}
  where $\xv_{-i} \in \mathbb{R}^{D - 1}$ is $\xv$
without the $i$-th dimension.
\end{definition}
We also note that the following holds by definition of the binary function:
\begin{equation}
  \begin{aligned}
    \gamma = \int_{\xv \in \X} b(\xv | \Xg) \frac{\mu(d\xv)}{\mu(\X)}.
  \end{aligned}
  \label{appendix:proofs:eq:binary-expectation-is-gamma}
\end{equation}
Then we first prove the following lemma:
\begin{lemma}
  The following holds:
  \begin{equation}
    \begin{aligned}
      \int_{x_i \in \X_i} q(x_i | \Xg)\frac{\mu(dx_i)}{\mu(\X_i)} = \gamma
    \end{aligned}
  \end{equation}
  \label{appendix:proofs:lemma:integral-of-marginalized-dist}
\end{lemma}
\begin{proof}
  By definition, the following equality holds:
  \begin{equation}
    \begin{aligned}
      \int_{x_i \in \X_i} q(x_i | \Xg)\frac{\mu(dx_i)}{\mu(\X_i)} =
      \int_{x_i \in \X_i} \int_{\xv_{-i} \in \X_{-i}} b(\xv | \Xg)
      \frac{\mu(dx_{-i})}{\mu(\X_{-i})}
      \frac{\mu(dx_i)}{\mu(\X_i)}.
    \end{aligned}
  \end{equation}
  Since the Lebesgue measure is a product measure
  and $b(\xv | \Xg) \geq 0$,
  the Fubini's theorem holds, and thus we obtain the following:
  \begin{equation}
    \begin{aligned}
      \mathrm{LHS} = \int_{\xv \in \X} b(\xv | \Xg) \frac{\mu(d\xv)}{\mu(\X)} 
      = \gamma~(\because \mathrm{Eq.~}(\ref{appendix:proofs:eq:binary-expectation-is-gamma})).
    \end{aligned}
  \end{equation}
  This completes the proof.
\end{proof}
Using this lemma, we prove Proposition~\ref{main:methods:proposition:hp-importance}.
\begin{proof}
  Since $b(\xv | \Xg)$ is a special version, such that $k(\xv, \xv^\prime) = \delta(\xv, \xv^\prime)$,
  of the $\gamma$-set PDF,
  the marginalization of $b(\xv | \Xg)$ is viewed as the marginalization
  of $p(\xv | \Xg)$ with a different scale.
  From Lemma~\ref{appendix:proofs:lemma:integral-of-marginalized-dist},
  the scale to equalize this marginalization is $\gamma\mu(\X_i)$,
  and thus the marginal $\gamma$-set PDF
  is computed as $p(x_i | \Xg) = q(x_i | \Xg) / (\gamma \mu(\X_i))$.
  Therefore, we obtain the following marginal variance:
  \begin{equation}
    \begin{aligned}
      \mathbb{V}_i &\coloneqq \mathbb{E}[(q(x_i | \Xg) - \gamma)^2] \\
      &= \mathbb{E}[(\gamma \mu(\X_i)p(x_i | \Xg) - \gamma)^2]\\
      &= (\gamma \mu(\X_i) )^2 \mathbb{E}\Biggl[
        \Biggl(p(x_i | \Xg) - \frac{1}{\mu(\X_i)}
        \Biggr)^2
        \Biggr]
    \end{aligned}
  \end{equation}
  and this completes the proof.
\end{proof}
As seen in the equation above,
the marginal variance is measured
via the L2 norm between the uniform PDF and
the marginal $\gamma$-set PDF.
We can rank each dimension by $\mathbb{V}_i$.


==> settings/labels-in-main.tex <==
\ifappendix
% Do nothing

\else

% Define the labels in the main sections
\customlabel{main:section:introduction}{1}
\customlabel{main:background:fig:similarity-conceptual}{1}
\customlabel{main:related-work:section}{2}
\customlabel{main:background:section}{3}
\customlabel{eq:l-and-g-trick}{4}
\customlabel{main:meta-learning-tpe:section}{4}
\customlabel{main:methods:eq:task-conditioned-acq-fn}{6}
\customlabel{main:methods:eq:task-similarity}{9}
\customlabel{main:when-does-method-fail:section}{4.3}
\customlabel{main:methods:alg:task-similarity}{1}
\customlabel{main:methods:theorem:gamma-set-converges}{1}
\customlabel{main:methods:alg:meta-tpe}{2}
\customlabel{main:methods:line:start-of-warm-start}{3}
\customlabel{main:methods:line:end-of-warm-start}{10}
\customlabel{main:methods:line:eps-greedy}{17}
\customlabel{main:methods:alg:meta-learn-tpe}{2}
\customlabel{main:methods:proposition:trivial-dims-not-matter}{2}
\customlabel{appx:case-I:fig:similarity-vs-convergence}{2}
\customlabel{appx:case-II:fig:high-dim-conceptual}{3}
\customlabel{appx:high-dim:eq:anova}{11}
\customlabel{main:high-dim:eq:reduced-kde}{13}
\customlabel{main:experiments:fig:hv-hpolib}{4}
\customlabel{main:experiments:section}{5}
\customlabel{main:experiments:fig:hv-nmt}{5}

% Start numberings of each data as if
% appendix takes over the numbering from the main section
\renewcommand\thefigure{\arabic{figure}}
\setcounter{figure}{5}  % start from 2
\renewcommand\thetable{\arabic{table}}
\setcounter{table}{0}  % start from 3
\renewcommand\thealgorithm{\arabic{algorithm}}
\setcounter{algorithm}{2}  % start from 4
\renewcommand\theequation{\arabic{equation}}
\setcounter{equation}{13}  % start from 5
\renewcommand\thetheorem{\arabic{theorem}}
\setcounter{theorem}{1}  % start from 5
\renewcommand\theproposition{\arabic{proposition}}
\setcounter{proposition}{2}  % start from 5

\renewcommand{\thesection}{\Alph{section}} 
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesection.\arabic{subsection}.\arabic{subsubsection}}

\fi

